It Is Time To Steer: A Scalable Framework for Analysis-driven Attack Graph Generation

Attack Graph (AG) represents the best-suited solution to support cyber risk assessment for multi-step attacks on computer networks, although their generation suffers from poor scalability due to their combinatorial complexity. Current solutions propose to address the generation problem from the algorithmic perspective and postulate the analysis only after the generation is complete, thus implying too long waiting time before enabling analysis capabilities. Additionally, they poorly capture the dynamic changes in the networks due to long generation times. To mitigate these problems, this paper rethinks the classic AG analysis through a novel workflow in which the analyst can query the system anytime, thus enabling real-time analysis before the completion of the AG generation with quantifiable statistical significance. Further, we introduce a mechanism to accelerate the generation by steering it with the analysis query. To show the capabilities of the proposed framework, we perform an extensive quantitative validation and present a realistic case study on networks of unprecedented size. It demonstrates the advantages of our approach in terms of scalability and fitting to common attack path analyses.

==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

This paper presented a new framework for AG-based systems addressing the problem of their scalability by leveraging progressive data analysis.
We designed two approaches to progressively generate statistically significant partial AGs (StatAG) and accelerate the generation based on the attack path query (SteerAG).
Additionally, it can better adapt to network changes (e.g., new connections or vulnerabilities in the network) without the need for recomputing the entire AG, a benefit that classic AG generation approaches lack.
We provided extensive experimental validation and showed a case study demonstrating the capability of the framework to (i) analyze networks whose size cannot be managed with existing solutions, and (ii) efficiently support common attack path analyses. The approach is orthogonal to the existing ones and can be used in their combination without loss of generality.
The entire framework and reproducible experiments are available as an open-source OSF repository at {\footnotesize \href{https://osf.io/9gctb/?view_only=b352d57cfd6149c99be2777bec05e1a5}{https://osf.io/9gctb/?view\_only=b352d57cfd6149c99be2777bec05e1a5}}.

In future works, we intend to 
i) Investigate the application of StatAG and SteerAG to the class of logical AGs,
ii) extend it to more heterogeneous risk models,
iii) apply advanced learning solutions, such as network representation learning, and iv) develop an interactive system to validate the approach in real scenarios with security experts.
